Model-driven Cluster Resource Management for AI Workloads in Edge Clouds

Since emerging edge applications such as Internet of Things (IoT) analytics and augmented reality have tight latency constraints, hardware AI accelerators have been recently proposed to speed up deep neural network (DNN) inference run by these applications. Resource-constrained edge servers and accelerators tend to be multiplexed across multiple IoT applications, introducing the potential for performance interference between latency-sensitive workloads. In this paper, we design analytic models to capture the performance of DNN inference workloads on shared edge accelerators, such as GPU and edgeTPU, under different multiplexing and concurrency behaviors. After validating our models using extensive experiments, we use them to design various cluster resource management algorithms to intelligently manage multiple applications on edge accelerators while respecting their latency constraints. We implement a prototype of our system in Kubernetes and show that our system can host 2.3X more DNN applications in heterogeneous multi-tenant edge clusters with no latency violations when compared to traditional knapsack hosting algorithms.

==> Makefile <==
#
# Makefile for acmart package
#
# This file is in public domain
#
# $Id: Makefile,v 1.10 2016/04/14 21:55:57 boris Exp $
#

PACKAGE=acmart


PDF = $(PACKAGE).pdf acmguide.pdf

all:  ${PDF} ALLSAMPLES


%.pdf:  %.dtx   $(PACKAGE).cls
	pdflatex $<
	- bibtex $*
	pdflatex $<
	- makeindex -s gind.ist -o $*.ind $*.idx
	- makeindex -s gglo.ist -o $*.gls $*.glo
	pdflatex $<
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $*.log) \
	do pdflatex $<; done


acmguide.pdf: $(PACKAGE).dtx $(PACKAGE).cls
	pdflatex -jobname acmguide $(PACKAGE).dtx
	- bibtex acmguide
	pdflatex -jobname acmguide $(PACKAGE).dtx
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' acmguide.log) \
	do pdflatex -jobname acmguide $(PACKAGE).dtx; done

%.cls:   %.ins %.dtx
	pdflatex $<


ALLSAMPLES:
	cd samples; pdflatex samples.ins; cd ..
	for texfile in samples/*.tex; do \
		pdffile=$${texfile%.tex}.pdf; \
		${MAKE} $$pdffile; \
	done

samples/%: %
	cp $^ samples


samples/$(PACKAGE).cls: $(PACKAGE).cls
samples/ACM-Reference-Format.bst: ACM-Reference-Format.bst

samples/%.pdf:  samples/%.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && pdflatex-dev $(notdir $<); done

samples/sample-xelatex.pdf:  samples/sample-xelatex.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && xelatex-dev $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && xelatex-dev $(notdir $<)
	cd $(dir $@) && xelatex-dev $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && xelatex-dev $(notdir $<); done

samples/sample-lualatex.pdf:  samples/sample-lualatex.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && lualatex-dev $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && lualatex-dev $(notdir $<)
	cd $(dir $@) && lualatex-dev $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && lualatex-dev $(notdir $<); done



.PRECIOUS:  $(PACKAGE).cfg $(PACKAGE).cls

docclean:
	$(RM)  *.log *.aux \
	*.cfg *.glo *.idx *.toc \
	*.ilg *.ind *.out *.lof \
	*.lot *.bbl *.blg *.gls *.cut *.hd \
	*.dvi *.ps *.thm *.tgz *.zip *.rpi \
	samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst \
	samples/*.log samples/*.aux samples/*.out \
	samples/*.bbl samples/*.blg samples/*.cut 



clean: docclean
	$(RM)  $(PACKAGE).cls \
	samples/*.tex

distclean: clean
	$(RM)  *.pdf samples/sample-*.pdf

#
# Archive for the distribution. Includes typeset documentation
#
archive:  all clean
	COPYFILE_DISABLE=1 tar -C .. -czvf ../$(PACKAGE).tgz --exclude '*~' --exclude '*.tgz' --exclude '*.zip'  --exclude CVS --exclude '.git*' $(PACKAGE); mv ../$(PACKAGE).tgz .

zip:  all clean
	zip -r  $(PACKAGE).zip * -x '*~' -x '*.tgz' -x '*.zip' -x CVS -x 'CVS/*'

documents.zip: all docclean
	zip -r $@ acmart.pdf acmguide.pdf samples *.cls ACM-Reference-Format.*

.PHONY: all ALLSAMPLES docclean clean distclean archive zip


==> README <==
This package provides a class for typesetting publications of the
Association for Computing Machinery.

Your TeX distribution probably includes the latest released version of
this package.  If you decide to install it yourself, please see the
Installation section of the User's Guide.

Please note that the version on Github is a development (or
experimental) version: please download it for testing new features.
The production version is the one on CTAN and ACM sites.


Changes

version 1.08    SIGPLAN reformatting (Matthew Fluet); bug fixes

version 1.09    SIGPLAN: revert caption rules (Matthew Fluet)

version 1.10    Bug fixes

version 1.11    Customization of ACM theorem styles and proof
                environment (Matthew Fluet).

version 1.12    Bug fixes and documentation updates.
                Footnotes rearranged.
                Option natbib is now mostly superfluous: the class
                makes a guess based on the format chosen.

version 1.13    Formatting changes: headers, folios etc.
                Bibliography changes.

version 1.14    Warn about undefined citation styles; move definitions
                of acmauthoryear and acmnumeric citation styles before
                use.

version 1.15    New structured affiliation command.
                New commands for acknowledgements.

version 1.16    Formatting changes for headers and footers.

version 1.17    Formatting changes for margins and lists.  Bug fixes.

version 1.18    Natbib is now the default for all versions.  A unified bib
                file is used for all styles.  Better treatment
                of multiple affiliations.

version 1.19    Include 'Abstract', 'Acknowledgements', and 'References'
                in PDF bookmarks.

version 1.20    Bug fixes, documentation updates

version 1.21    Bibliography changes: added arXiv, some cleanup

version 1.22    Bibliography changes for Aptara backend; should be
                invisible for the users.

version 1.23    Added PACM PL journal option.

version 1.24    Added IMWUT journal option.

version 1.25    Updated PACMPL journal option.

version 1.26    Bug fixes

version 1.27    Bug fixes

version 1.28    Bug fixes: natbib=false now behaves correctly.

version 1.29    Documentation changes.  Head height increased from 12pt to 13pt.
                Removed spurious indent at start of abstract.
                Improved kerning in CCS description list.

version 1.30    Bibtex style now recognizes https:// in doi.
                Added \frenchspacing.
                \department now has an optional hierarchy level.
                Switched to T1 encoding
                Updated IMWUT and PACMPL

version 1.31    Changed default year and month to the current ones
                (thanks to Matteo Riondato)
                Table of contents now works
                Marginalia now work in all formats
                New command \additionalaffiliation
                Documentation changes

version 1.32    New DOI formatting.
                Format siggraph is now obsolete, and sigconf
                is used instead.
                New proceedings title: POMACS.

version 1.33    New option `timestamp' (Michael D. Adams)
                New option `authordraft'
                Documentation updates
                Bug fixes
                We now use Type 1 versions of Libertine fonts even with XeTeX.
                New hook acmart-preload-hook.tex (wizards only!)
                Added new options `obeypunctuation' for \affiliation command
                Added SubmissionID
                Added right line count ruler for two-column formats
                Added workaround for Adobe Acrobat bugs in selection
                Added eid field to the bibliography

version 1.34    Deleted DOI from doi numbers
                Changed bibstrip formatting
                The command \terms is now obsolete
                The rulers in review mode now have continuous numbering

version 1.35    Author-year bib style now uses square brackets.
                Changed defaults for TOG sample
                Price is suppressed for usgov and rightsretained modes.
                Bugs fixed

Version 1.36    Bug fixes
                Moved PACMPL to acmlarge format
                New journal: PACMHCI
                Added the possibility to adjust number of author
                boxes per row in conference formats

Version 1.37    Reduce list indentation (Matthew Fluet)

Version 1.38    Increase default font size for SIGPLAN

Version 1.39    Added \authornotemark commmand

Version 1.40    Bibliography changes
                Added processing of one-compoment ccsdesc nodes
                Bug fixes.
                Made the height a multiple of \baselineskip + \topskip
                Added cleveref
                We no longer print street address in SIGs

Version 1.41    Rearranged bib files
                Added new badges

Version 1.42    Deleted ACM badges
                Bug fixes

Version 1.43    Bug fixes

Version 1.44    Bug fixes.
                Empty DOI and ISBN suppress printing DOI or ISBN lines
                Separated theorem code into acmthm.sty, loaded by default.
                Article number can be set for proceedings.
                New commands: \acmBooktile, \editor.
                Reference citation format updated.

Version 1.45    Workaround for a Libertine bug.  Thanks to LianTze Lim
                from Overleaf

Version 1.46    Bug fixes for bibliography: label width is now calculated
                correctly.
                All PACM now use screen option.  This requires etoolbox.
                Added subtitle to ACM reference format.
                Now acmart is compatible with fontspec.
                \thanks is now obsolete.  The addresses are automatically
                added to the journal version; this can be overriden with
                \authorsaddresses command.
                Deleted the rule at the end of frontmatter for all formats.
                Deleted new line before doi in the reference format.
                Reintegrated theorem code into acmart.dtx (Matthew Fluet)

Version 1.47    New journal: THRI

Version 1.48    Bug fixes
                Review mode now switches on folios
                Code prettying (Michael D. Adams)
                Bibliography changes: @MISC entries no longer have a
                separate date
                Sigch-a sample bibliography renamed
                Bib code cleanup (Zack Weinberg)
                Acmart and version info are added to pdfcreator tag
                \citeyear no longer produces parenthetical year
                Added initial support for Biblatex (Daniel Thomas)
                Added support for IW3C2 conferences

Version 1.49    New jorunal:  DTRAP

Version 1.50    Changes in iw3c2w3 and iw3c2w3g

Version 1.51    Journal footers now use abbreviated journal titles.
                Corrected the bug with acmPrice.
                Do not show price when copyright is set to iw3c2w3 and iw3c2w3g.
                The package now is compatible with polyglossia (Joachim Breitner).
                Slightly reworded copyright statements.

Version 1.52    Another rewording of licenses

Version 1.53    New journals: PACMCGIT, TIOT, TDSCI

Version 1.54    New option: 'nonacm' (Gabriel Scherer)
                Deleted indent for subsubsection (suggested by Ross Moore)
                Suppressed some obscurious warning in BibTeX processing
                Suppressed hyperrerf warnings (Paolo G. Giarrusso)
                New code for sections to help with accessibility patches
                (Ross Moore)
                Submission id, if present, is printed in anon mode
                Bug fixes

Version 1.55    Bug fixes
                Font changes for SIGCHI table captions

Version 1.56    Bug fixes
                Added \flushbottom to two column formats (Philip Quinn)
                The final punctuation for the list of concepts
                is now a period instead of a semicolon (Philip Quinn)
                New command \Description to describe images for visually
                impaired users.

Version 1.57    Change of \baselinestretch now produces an error
                Booktabs is now always loaded
                Added option `balance' to balance last page in two-column mode
                E-mail is no longer split in addresses
                New samples (Stephen Spencer)

Version 1.58    Suppressed spurious warnings.
		New journal:  HEALTH.
		TDSCI is renamed to TDS.

Version 1.59    Now a journal format can be used for conference proceedings
		All samples are now generated from the same .dtx file
		Bug fixes

version 1.60    New option: urlbreakonhyphens (thanks to Peter Kemp)
		Smaller header size for acmsmall

Version 1.61    Bug fixes
                New bibtex types for artifacts

Version 1.62    Documentation update
		New journal: TELO
		Bug fixes

Version 1.63	New journals: TQUANT, FACMP

Version 1.63a   Moved TQUANT to TQC

Version 1.64    Produce error if abstract is entered after maketitle
		(previously abstract was silently dropped)
		Bug fixes for line numbering

Version 1.65   Bug fixes
	       New journal: DGOV
	       DTRAP and HEALTH are now using acmlarge format

Version 1.66   Bug fixes
	       BibTeX change:  location is now a synonym for city (Feras Saad) 
	       ACM reference format is now mandatory for papers over one page.
	       CCS concepts and keywords are now mandatory for
	       papers over two pages.
	       Authors' addresses are mandatory for journal articles.

Version 1.67   Urgent bug fixes:
	       BibTeX style bug fixed (Michael D. Adams)
	       Sigplan special section bugfix

Version 1.68   Bug fixes
               BST now recognizes words `Paper' or 'Article' in
	       eid or articleno

Version 1.69   Bug fixes
	       Compatibility with LaTeX 2020-02-02 release

Version 1.70   Title change for ACM/IMS Transactions on Data Science
               Bug fixes for bibliography


Version 1.71   Bug fixes
               Formats sigchi and sigchi-a are retired
	       Bibliography formatting changes for @inproceedings entries
	       having both series and volume
	       LuaLaTeX now uses the same OTF fonts as XeLaTeX

Version 1.72   Bug fixes.  Better handling of metadata.

Version 1.73   Bug fixes
	       The elements institution, city and country are now obligatory
	       for affiliations

Version 1.74   Bug fixes.  A regression introduced in the font changes
	       is reverted.

Version 1.75.  \country is now obligatory for addresses.
	       Added \AtBeginMaketitle

Version 1.76.  Added many journal abbreviations to the bst.
	       New experimental option: pbalance
	       ORCID linking code

Version 1.77.  Changed the way to typeset multiple affiliations (Christoph Sommer)

Version 1.78.  Documentation update.
	       Magic texcount comments for samples.
	       Title page now is split if there are too many authors
	       Bug fixes.

Version 1.79.  Fixed pages with index
	       (https://github.com/borisveytsman/acmart/issues/440)
	       Updated information for TAP, TCPS, TEAC

==> imgs-latex/Concurrency-Effect.tex <==
\begin{figure*}[t]%
    \centering
    \subfloat[Batching - Jetson nano]{{
        \includegraphics[width=0.32\linewidth]{imgs/nano_batch_throughput.pdf} 
        \label{fig:nano-conc-batch}
    }}%
    \subfloat[Batching - Nvidia 1080]{{
        \includegraphics[width=0.32\linewidth]{imgs/1080_batch_throughput.pdf} 
        \label{fig:1080-conc-batch}
    }}%
     \subfloat[MPS - Nvidia 1080]{{
        \includegraphics[width=0.32\linewidth]{imgs/1080_MPS_throughput.pdf}
        \label{fig:1080-conc-mps}
    }}%
    \caption{Throughput change with Parellelism  }%
\label{fig:concurrency-effect}%
\end{figure*}


==> imgs-latex/TPU-effect.tex <==
\begin{figure}%
    \centering
    \subfloat[Single Request]{{
        \includegraphics[width=0.45\linewidth]{imgs/placeholder.png} 
    }}%
    \subfloat[Multiple Requests]{{
        \includegraphics[width=0.45\linewidth]{imgs/placeholder.png} 
    }}%
    \caption{TPU Inference}%
\label{fig:tpu-effect}%
\end{figure}

==> imgs-latex/fig2-.tex <==
 \begin{figure}[t]
	\centering
	\subfloat[]{
		\includegraphics[width=0.4\textwidth]{imgs/inference_as_a_service.pdf}\label{fig:inference_as_a_service}
	} \hspace*{0.2in}
	\subfloat[]{
		\includegraphics[width=0.26\textwidth]{imgs/user_trained.pdf}\label{fig:user_trained}
	}
	\caption{Two-tiered edge application architecture. (a) Inference as a service application with multiple frontend containers shares a single backend. (b) User-trained models use a one-to-one mapping of frontend and backend containers.}
	\label{fig:two_tier_arch}
\end{figure}

==> imgs-latex/placement_1080.tex <==
\begin{figure*}[h]%
    \centering
    \subfloat[AI-as-a-Service]{{
        \includegraphics[width=0.4\linewidth]{imgs/sim_MAAS.pdf} 
        \label{fig:placement_1080_MaaS}
    }}%
    \subfloat[User-Trained Models]{{
        \includegraphics[width=0.4\linewidth]{imgs/sim_USER.pdf} 
        \label{fig:placement_1080_user}
    }}%
    \caption{Model placement on Discrete GPU}
\label{fig:placement_simulation}%
\end{figure*}

==> src/architecture.tex <==
%\section{Tiered Architecture For Edge Applications}
\section{System Design and Goals}
\label{sec:tiered}

%\textcolor{red}{Depending on the changes to the problem statement, I feel like we need to motivate the two tiered arch either here or in the previous section. I think one way would be to start this section with the problem statement, and then weave in the text what we plan to do in the section.}


%\input{imgs-latex/fig2}

The overall goal of our work is to design an edge resource management system to multiplex IoT applications on to a cluster of edge nodes with accelerators. Each edge node is a commodity server with one or more accelerators such as GPU or TPU. Each IoT application  is designed to process sensor data generated by its corresponding IoT device and is assumed to employ a DNN model for this data processing. Each application has response time  requirements, which is specified as   $R_i$, the desired mean response time for application $i$.  The request rate (i.e., workload) seen by the application is stochastic due to the stochastic nature of sensor data generation. Let $\lambda_i$ denote the worst-case request rate (i.e., upper bound) that will be seen by application $i$. The goal of our system is to provide  guarantees on request processing latency---by ensuring that requests will see a mean response time of $R_i$ under the worst case workload rate of $\lambda_i$ with high probability.  {\em Note that the guarantees are soft (probabilistic) guarantees---analogous to service time guarantees given to cloud-based web applications \cite{Urgaonkar2005}---rather than hard real-time ones.}   Since each edge node may run multiple applications, the system should ensure the desired  latency $R_i$ for each co-located application. As more applications are mapped onto a node, the  load on the system  will increase, causing the response time seen by each application to degrade. Thus, the system should limit the number of applications running on each node so that the response times do not degrade beyond the desired value $R_i$, while also attempting to run as many applications on each nodes as possible to maximize resource sharing. 

Each IoT application is assumed to be virtualized using OS containers and uses a two-tier container architecture (similar to multi-tier web applications \cite{Urgaonkar2005}). See Figure \ref{fig:two_tier_archiecture}.  The front-end container receives requests (in the form of sensor data such as camera images) and perform pre-processing of this data as needed before handing it to the backend tier. The backend container houses the DNN model for the application and performs inference on the request by executing the model on the underlying edge accelerator. Thus, the front-end container performs CPU processing on the request, while the backend performs GPU or TPU processing. The overall response time of a request $R$ is the sum of the response times of the two tiers. That is $R=R_{front}+R_{back}$, which also translates to $R=R_{cpu} + R_{gpu/tpu}$, where $R_{cpu}$ and  $R_{gpu/tpu}$ denote the response time for CPU and GPU/TPU execution.  The goal of the system is to ensure $R_{cpu} + R_{gpu/tpu} \leq R_i$. 


To ensure performance isolation, OS container mechanisms (e.g.,\texttt{cgroups} in Linux) are used to allocate a slice of CPU, network and memory resources to frontend and backend containers.   Since no such isolation mechanisms are available for accelerators such as edge GPUs and TPUs,  our system uses two methods to reduce interference. 
First, each backend container implements  a token bucket rate regulator \cite{token-bucket} to ensure that the request rate of each application is limited to no more than $\lambda_i$ requests/s. Second, our algorithms discussed  in \S \ref{sec:slo} limit the number of applications running on each node to ensure that response time guarantees are met. 

Assuming such two-tier applications, our system supports two types of IoT applications.
\subsection{AI-as-a-Service}
In the simplest case, the edge cluster can provide IoT applications with a list of pre-trained models and ask the application to choose one that is best suited for its inference needs.  Once the application specifies a  model, the edge cluster can provision a backend cointainer   containing that pre-trained model. We refer to this approach as \emph{AI-as-a-Service (AIaaS)} since the cloud supports inference processing as a service using pre-trained models for common inference tasks. For example, as noted in \S \ref{sec:background}, pre-trained DNN models such as Yolo, ResNet, and Inception have become popular for inference tasks such as classification and recognition.
%For example, \textcolor{red}{Ahmed: Move a much more concise version of Table 1 here, or move the entire Table to the Appendix. It does not break the flow of the paper, and is not important to the rest of the understanding.}  Table \ref{tab:models} lists popular pre-trained models that can be used for image or video analytics tasks such as object detection and recognition. 
The advantage of the AI-as-a-Service approach is that it maximizes resource sharing---if multiple applications choose the same underlying pre-trained model, the edge cluster can host these applications on the same edge server, allowing them to share container and hardware resources on the server. This is done by  mapping \emph{multiple} frontend containers corresponding to each application  onto a \emph{single} backend container, as depicted in Figure \ref{fig:two_tier_archiecture}.  The backend container runs a common DNN model that is requested by these applications .


\subsection{User-trained Models}
While pre-trained deep learning models provide good accuracy for a range of common tasks, some applications may have special needs that require training a model from scratch or retraining a DNN model with additional data. In this case, the application provides it own custom-trained DNN model.  We assume that the application provides its custom model in 
a standard hardware-agnostic format such as PMML, PFA, or ONNX \cite{Ferguson2019}, which is then compiled to native form to run on a GPU or TPU.    The application will then comprise a front-end container that  is mapped onto its own backend container containing the DNN (see Figure \ref{fig:two_tier_archiecture}).  Note that multiple backend containers belonging to different applications can still run on, and share, a single edge accelerator. 
  

%\input{imgs-latex/Architecture}

 In the following sections, we address two key design questions: (1) How can we estimate the response time of a DNN-based IoT application running on a shared server with other applications? (2) How can we use this analytic model to design co-location and migration techniques to maximize edge sharing while meeting response time guarantees?

 %In such cases, the edge cluster needs to support hosting of custom DNN models that are trained and provided by the users for their edge applications. Since training frameworks support standardized model formats, we assume that the user supplies a custom-trained  model in a standard hardware-agnostic format such as PMML, PFA, or ONNX \cite{Ferguson2019} to the edge cloud. The edge cluster can then compile this model to a native form (depending on the hardware architecture of the edge node accelerator) and then provision the model using a container on one of these nodes. Once provisioned, the user's device can submit  requests to the edge node for performing deep learning inference using the model. 





%Given the above background, consider an edge  cluster of $N$ servers that comprises commodity components (CPU, memory, disk) and a heterogeneous mix of edge accelerators for DNN inference.  Each DNN inference application is assumed to specify its latency needs in terms of a \emph{service level objective} (SLO), which in this case is the mean inference response time. The mean  inference response time is assumed to include both CPU response time as well as the GPU/TPU response time on the edge server incurred during request processing. We also assume that each application specifies the worst-case request arrival rate $\lambda$ for which edge resources need to be provisioned. Our goal is to design a system and resource management techniques that  maximize cluster utilization through multi-tenancy (where each server run multiple tenant applications) while respecting the SLO needs of each application and minimizing interference between co-located tenants.


%To address this goal, we present \emph{Ibis}, a system for managing multi-tenant applications running on a cluster of edge servers with heterogeneous DNN accelerators. Ibis uses a two-tier container architecture and analytic models to limit interference between tenants and uses intelligent resource management algorithms to meet SLO objectives and handle dynamic workloads. This section discusses Ibis' two-tiered  architecture for DNN inference applications that (i) enables applications to run arbitrary application code on edge servers, (ii) enables secure sharing of hardware accelerator resources across multiple tenants, and (iii) limits interference between co-located tenants.  It also facilitates flexible resource management policies for different cloud hosting strategies. 



%\subsection{Hosting Inference Applications}
%Ibis is designed to host two types of DNN inference applications---depending on whether the user choose a DNN from a  library of pre-trained DNN models or supplies a custom-trained DNN model for their application.

%As noted in \S \ref{sec:background}, many frameworks support a library of pre-trained models for DNN inference. Alternatively, users can also choose to train their own custom DNN model for their applications. 
%advances in AI have led to the emergence of easy to use frameworks such as TensorFlow and PyTorch that make is easy for users to train a DNN models that is tailored for their needs. Many frameworks also offer a library of pre-trained models that require no training effort from users---users can simply download such a pre-trained model, some of which are shown in Table \ref{tab:models}, and immediately deploy it for inference processing. 
%Consequently, depending on whether the user chooses an off-the-shelf pre-trained model or trains a custom-trained model for their  inference needs, an edge cloud can use two different strategies to host and execute these DNN model based applications. 

%There has been significant advances in deep learning that have resulted in a range of Deep Neural Networks (DNNS) for various tasks such as classification, object recognition, etc. Due to the increase in the availability of labeled datasets, the research community, and industry have produced numerous tools for training such models (e.g., TensorFlow, PyTorch, Caffe, etc.) as well as pre-trained models for specific tasks. Moreover, many modeling frameworks provide a “model zoo” of pre-trained models, such as models shown in Table \ref{tab:models}, that allows users to simply download a model and start using it for deep learning inference by sending input requests. Alternatively, users can use the deep learning framework to train these models from scratch using custom training datasets or edit and retrain a pre-trained model using additional data, known as transfer learning.

%Consequently, depending on whether users choose an off-the-shelf pre-trained model or a custom-trained model for their IoT inference needs. An edge cloud can provide two types of model hosting strategies. 
%\subsubsection{AI-as-a-Service}
%In the simplest case, an edge cloud can provide users with a list of pre-trained models and ask the user to choose one that is best suited for their inference application.  Once the user specifies a  model, the edge cloud can provision a container VM containing that pre-trained model. We refer to this approach as \emph{AI-as-a-Service (AIaaS)} since the cloud supports inference processing as a service using pre-trained models for common inference tasks. For example, as noted in \S \ref{sec:background}, pre-trained DNN models such as Yolo, ResNet, and Inception have become popular for inference tasks such as classification and recognition.
%For example, \textcolor{red}{Ahmed: Move a much more concise version of Table 1 here, or move the entire Table to the Appendix. It does not break the flow of the paper, and is not important to the rest of the understanding.}  Table \ref{tab:models} lists popular pre-trained models that can be used for image or video analytics tasks such as object detection and recognition. 
%The advantage of the AI-as-a-Service approach is that it maximizes resource sharing---if multiple users choose the same underlying pre-trained model, the edge cluster can host these users on the same edge server, allowing them to share container and hardware resources on the server, which is desirable in resource-constrained edge settings. In \S \ref{sec:two-tier}, we discuss how such sharing can be done securely across untrusted applications belonging to different users.



%In many cases, a pre-trained deep learning model may suffice for processing inference requests from IoT devices. In this case, the edge cloud can provide users with a list of popular pre-trained models and have them choose one that fits their needs. The edge cloud then provisions this pre-trained model on an edge node, and users can start using this provisioned model by sending inference requests. We refer to this approach, by Supporting popular pre-trained models, as Model-as-a-Service (MaaS). This approach simplifies the process for end-users who no longer have to provide a model and can simply choose a supported model. This approach is also attractive to the edge cloud providers since it maximizes resource sharing for popular models - A single provided model can support inference requests from multiple devices. For example, a popular model such as MobileNet can be provisioned on an edge node and provide object recognition (inference) services to multiple home security cameras from different users; doing so maximizes sharing benefits, especially in resource-constrained edge clusters.

%\subsubsection{User-trained Models}
%While pre-trained deep learning models provide good accuracy for a range of common tasks, some users may have special needs that require training a model from scratch or retraining a DNN model with additional data. In such cases, the edge cluster needs to support hosting of custom DNN models that are trained and provided by the users for their edge applications. Since training frameworks support standardized model formats, we assume that the user supplies a custom-trained  model in a standard hardware-agnostic format such as PMML, PFA, or ONNX \cite{Ferguson2019} to the edge cloud. The edge cluster can then compile this model to a native form (depending on the hardware architecture of the edge node accelerator) and then provision the model using a container on one of these nodes. Once provisioned, the user's device can submit  requests to the edge node for performing deep learning inference using the model. 

%\textcolor{red}{Ahmed: Is the next para important?}
%We note that the interface provided to the user's devices is identical in both pre-trained and user-trained models, since both approaches involve deploying a container VM comprising the DNN model for processing user requests. The only difference is that the latter requires the user to supply the model to be executed inside the container, while the former involves choosing from a  list of supported (pre-trained) models.

%\subsection{Two-Tier Virtualized Architecture}
%\label{sec:two-tier} 
%\textcolor{red}{ This subsection is extremely long. }
%Both AIaaS and user-trained DNN hosting involves executing inference models inside containers, with multiple tenant applications running on an edge server. A standard approach for multiplexing hardware resources across multiple
%untrusted applications is to use virtualization \cite{Xen2003,cgroup}. However, edge accelerators typically do not provide hardware support for virtualization, and their rudimentary multiplexing features complicate the design of OS schedulers
%for resource partitioning across applications. This lack of isolation mechanisms raises two concerns. First, sinceeach co-located tenant will load its DNN model onto the hardware GPU or TPU for  execution and there is no memory isolation on the accelerator; doing so exposes a DNN model belonging to one customer to others---a malicious user  can \emph{steal} another's customers model from GPU or TPU memory or corrupt the DNN model by overwriting another user's GPU memory area.  Second, each executing tenant can issue DNN inference requests at arbitrary rates, causing  accelerator overload and performance degradation for all co-located tenants.  To address these security and isolation concerns, Ibis employs a two-tier container architecture for each DNN inference application (similar to the multi-tier architecture \cite{Urgaonkar2005} used by web applications). Ibis' tiered architecture ensures safety and isolation, while allowing flexibility of running arbitrary user code within each application and sharing of edge resources across multiple tenants.




%The frontend tier container, depicted in Figure \ref{fig:two_tier_archiecture}, is fully under  user control and can run any custom user code that is needed by the application (e.g., to receive data over the network from a phone or IoT device and to pre-process the data prior to submitting it to the model for inference). In contrast, the backend tier container  is under the cloud provider's control, and users do not have access to the container or processes running inside them, except through a well-defined network interface to submit a request from the frontend container for inference. The backend container executes the DNN model (e.g., using a run-time framework such as TensorRT or TensorFlow) and has direct access to the hardware accelerator during inference processing.  Multiple backend containers may run on an edge server. However, since all such containers are under the cloud provider's control with no customer access, they are assumed to be trusted; thus, they can share the hardware accelerator and its memory  without security concerns. Frontend containers, which run user code, are prohibited from directly accessing the hardware accelerator using OS access control mechanisms (e.g.,\texttt{cgroups} in Linux).  

%Each backend container implements  a token bucket rate regulator \cite{token-bucket} to ensure isolation by limiting the rate at which frontend containers issue inference requests. Further,  the cloud provider can control how many applications (and backend containers) to run on each server to avoid server overload and meet  SLO objectives. To ensure that backend containers run code that is trustworthy, the cluster manager constructs each backend container for edge applications.  Users supply DNN models in standard form (e.g., ONNX), and the cluster compiles it into native form for the GPU or TPU; the compiled model and a standard run-time such as TensorRT are loaded into the backend container.


%However, hosting a user's edge application code as well as the model run-time inside a single container raises isolation and security concerns---since the container needs direct access to the hardware accelerator to execute the DNN model. Since multiple containers can share an edge server, and each such container  loads its model onto the hardware GPU or TPU for faster execution, doing so exposes a model belonging to one customer to others. Lack of isolation mechanisms on hardware accelerators means that a malicious user  can \emph{steal} another's customers model from GPU or TPU memory or corrupt the model by overwriting another user's GPU memory area. 

%The standard approach for avoiding such problems has been to provide isolation by \emph{virtualizing} hardware resources and exposing a virtualized resource, rather than the physical one, to each VM \cite{Xen2003}. The use of virtualized resources \emph{sandboxes}  the VM and its application and prevents it from accessing memory or data belonging to a different user. While techniques to virtualize traditional resources such as CPU and memory are well known \cite{Xen2003}, new hardware such as edge accelerators often lack  hardware support for virtualizing these resources. An alternate approach to virtualization is to use resource partitioning mechanisms that provide similar isolation. This is the approach used in  OS container virtualization, where a resource is partitioned across containers, and OS level schedulers are used to enforce such partitioning \cite{rajkumar2008,Hanafy2019}. For example, the \texttt{cgroup} mechanism in Linux \cite{cgroup} can be used to partition CPU cores and RAM, and allocate each slice to a different container.  However, hardware accelerators provide rudimentary multiplexing mechanisms, it at all, making it challenging to implement OS-level resource partitioning and scheduling techniques.


%Due to the challenges in virtualizing edge hardware accelerators or providing resource partitioning mechanisms, we propose a novel method that uses tiering to achieve isolation across applications while enabling resource sharing.  Our approach involves running edge applications using two containers rather than a single one. These containers form a two-tiered architecture (similar to the multi-tier architecture \cite{Urgaonkar2005} used by web applications). The frontend container, depicted in Figure \ref{fig:two_tier_arch}, is fully under  user control and runs any custom code that is needed by the application (e.g., to receive data over the network from a phone or IoT device and to pre-process the data prior to submitting it to the model for inference). The backend tier container, on the other hand,  is under the cloud provider's control and users do not have access to the container or processes running inside them, except through a well-defined network interface to submit a request from the frontend container for inference. The backend container executes the DNN model (e.g., using a run-time framework such as TensorRT or TensorFlow) and has direct access to the hardware accelerator during inference processing.  Multiple backend containers may run on an edge server, and all of them will have access to the hardware accelerator. However, since all such containers are under the cloud provider's control with no customer access to these containers, they are assumed to be trusted; thus they can share the hardware accelerator and its memory  without security concerns. Frontend containers, which run user code, are prohibited from directly accessing the hardware accelerator using OS access control mechanisms (e.g.,\texttt{cgroups} in Linux).  The cloud provider can control how many backend containers to run on each server to ensure adequate level of sharing while also respecting SLO objectives. The backend container can also implement a rate regulator such as a token bucket \cite{token-bucket} to ensure isolation by limiting the rate at which frontend containers issue inference requests.  


  

%A key assumptions in our approach is that backend containers are trusted since they are under cloud provider's control. The cloud provider needs to ensure that only trustworthy code is running inside each such container. To do so, we assume that each backend container is constructed by the  cloud provider on behalf of each application---frontend container of an application is assumed to be supplied by the customer (e.g., in the form of a docker image), and thus, can run arbitrary code. An application, however, does not supply its backend container. Instead, it specifies the DNN model that is to be used in the backend (e.g., for AI-as-a-service) or supplies the DNN model in a standard format (e.g., ONNX) in case of a user-trained model. In either case, the cloud provider takes the specified model in standard form and compiles it into native form for the GPU or TPU. It then constructs the backend container for the application using this compiled model and a run-time system to execute the model. By ensuring it uses its own software components to construct the backend container on behalf of each application, a cloud provider can ensure the backend tier runs code that will be well behaved.

% \textcolor{red}{Ahmed: Suggest to remove all the two paragraphs below, moving the figures earlier since we already sort of repeat things here.}
%  Such a two-tiered architecture provides both \emph{flexibility} and \emph{isolation}. A customer can still run their own custom code for the edge application in the frontend container, which provides flexibility. Inference processing is performed by the backend containers, which remain under cloud provider control ensuring secure sharing of hardware accelerator resources.
 
 

 %Such a two-tiered architecture is general and can be adapted to various edge scenarios. In case of AI-as-a-service, \emph{multiple} frontend containers are mapped onto a \emph{single} backend container, as depicted in Figure \ref{fig:two_tier_archiecture}.  The backend container runs a DNN model that is requested by multiple applications, and these applications can transparently share a single backend that executes this model. In contrast, edge applications with user-trained DNNs comprise a frontend container mapped onto their own backend container containing the DNN (see Figure \ref{fig:two_tier_archiecture}).  In either case, each edge server and accelerator can run one or more backend containers, each of which has one or more frontend containers mapped on it, yielding different degrees of multi-tenancy. 

 

%The standard model for running applications on the cloud is to employ virtualization, where the application runs inside a virtual machine, and multiple VMs belonging to different users may reside on the same server but are securely isolated from one another. This is feasible since all server resources (CPU, Memory, and Network Interface) are virtualized and can be shared across resident VMs.

%However, newer hardware resources such as TPU and GPU accelerators are harder to virtualize than traditional resources such as a CPU; we present a two-tied virtualized architect to enable sharing of edge resources while providing isolation from other users.

%Our Architecture depicted \ref{fig:architecture} is based on OS containers, a lightweight virtualization technology. We use two layers of containers, a frontend container that runs user code and a backend container that contains the model and performs inference. frontend containers are under user control, and users can use them to perform preprocessing over the IoT data prior to submitting them to the backend container for inference. backend containers are under cloud provider control, and users do not get direct access to them except via a well-defined interface to invoke the deep learning inference on the resident model.

%This separation is necessary for isolating cloud users from one another since newer edge devices are not amendable to virtualization, and even edge GPU pose challenges to virtualization, the backend container will need direct access to the physical accelerator hardware. Also, devices such as GPUs don’t provide any isolation, which means that if multiple DNNs are loaded on a device, a user process can modify any other DNN in addition to its own. This is undesirable when running a third-party cloud application. However, by ensuring that the backend containers remain under the cloud provider’s control, we can ensure that all backend containers remain well behaved. On the other hand, frontend containers don’t have/need access to the hardware accelerator resource except through the interface provided by the backend containers. 

%Thus, our two-tier architecture, which is similar to multi-tier architecture user by cloud-based web applications, retains flexibility, by allowing users to run arbitrary preprocessing steps in the frontend container while ensuring securing sharing through the backend container that runs deep learning inference under cloud providers control.

%More importantly, such a two-tier abstraction can accommodate a range of scenarios for edge inference.  For example, multiple frontend containers belonging to different users can be mapped to the same backend container running a particular model. This is useful in MaaS hosting, where multiple users choose the same popular model for their inference needs. Sharing the same backend container obviates the need to load redundant copies of the same model, one for each user. Since the backend container is under the cloud provider’s control, users remain oblivious that their frontend container shares the same backend. 

%In addition to the many-to-one mapping, a one-to-one mapping allows each frontend to have its own backend containers, which is needed for running user-supplied models, where each model runs on its own backend container.

%Another possibility is a mix, where the edge node runs multiple backend containers, each contains a different model, but each backend serves multiple frontend containers. This mapping is useful for running multiple MaaS models on a node where the incoming traffic does not justify running a single backend container per node. Such mappings are also useful for running fused models which we discussed in section 2.


==> src/experiment.tex <==
\section{Experimental Evaluation}

%We now describe our experimental setup, followed by a detailed validation of our queuing models, and a thorough evaluation of Ibis.

In this section, we experimentally evaluate our model-driven approaches to answer two key questions. (1) How effective are our analytic models at predicting application response times in shared edge servers? (2) How effective are our resource management algorithms for providing response time guarantees? 

\subsection{Experimental Setup}
%In this section we describe the setup we use to validate our models, and to test our proposed model based load management algorithms.






%\subsubsection{Cluster Setup} We use a custom-built edge cluster of ten nodes (see figure \ref{fig:cluster} in Appendix \ref{apx:cluster}) each comprising a Jetson Nano GPU, 4 GB of RAM and quad-core ARM processor. We use a similar ten node cluster equipped with USB edge TPUs for our TPU experiment. The cluster also contains a Dell PC with 3.2 GHZ i7-8700 processor, 16 GB RAM, and Geforce-GTX-1080 GPU. All machines are connected via a gigabit ethernet switch and run Linux Ubuntu 18.04. Further, each Jetson Nano runs CUDA 10.2, cuDNN 8, and TensorRT 7.1.3 while the PC runs CUDA 11, cuDNN 7.6.5, and Jetson 7.1.3. All machines are virtualized using Docker 19 and managed by Kubernetes 11; gRPC 1.31 is used for inter-communication.

\subsubsection{Trace Workloads} The sensor trace workload for each IoT application is constructed using a sequence of images from the ImageNet dataset \cite{imagenet}.   Further, to construct a mix of IoT applications  to run on the edge cluster,  we use the public Azure trace \cite{Azure-traces} to construct a realistic mixes of containerized applications of varying sizes.  To do so, we analyze the distribution of VM sizes  (CPU utilization and memory footprint) 
in the Azure trace and use them to generate the utilization and model size of our DNN-based applications. We categorize VMs as small ($<$2GB), medium (2-8GB), and large ($>$8GB) and find that proportions of small, medium and large applications is 47\%, 33\%, and 20\% respectively.   The mix of small, medium and large DNN models housed on the edge cluster is chosen in the same proportion.  Finally, models in the same category are chosen evenly. 






==> src/introductionv1.tex <==
\section{Introduction}

Recent hardware advances have resulted in numerous hardware accelerator for edge devices to accelerate Machine Learning (ML) inferencing at the edge. For instance, Intel Movidius Vision Processing Units (VPU) \cite{movidius-vpu}, Google Edge TPU \cite{Cass2019TakingAT} and Nvidia Jetson embedded GPU \cite{nvidia-jetson} all claim to significantly speedup ML inferencing on edge nodes.

Since edge resources are naturally more resource-constrained than cloud resources available in large cloud data center. It is expected that such edge accelerator will be widely deployed on edge nodes for more efficient edge processing of ML inference requests from IoT devices. 

Since edge clusters are more resource constrained, dedicating an edge accelerator to a single IoT device may not be feasible --- sharing each edge node and its accelerator across multiple inference model is desirable. 

However, the latency-sensitive nature of the workload requires such resource sharing to be done judiciously --- if too many workloads are mapped onto a node, the inference latency may be unacceptably high and if too few workload share a node, precious node resources will be underutilized. Thus, resource sharing policies will need to consider both performance and utilization when multiplexing node resources across multiple devices and their workloads. 

While sharing of cloud servers across multiple users through Virtual Machine (VM) placement and analytic modeling is well understood, these techniques do not apply to sharing edge server resources. This is primary because sharing of processing resources (e.g. CPU) on cloud server is well-understood through time sharing, while hardware accelerators on edge nodes are hard to share. Some devices are only capable of sequential processing when serving requests from multiple DL models; Others are capable of process sharing while still can provide fine parallelism when serving multiple inference requests. 

These hardware differences imply that, unlike CPU models, no single analytic model or a single resource sharing policy can be applied when sharing edge resources. The difference need to be explicitly captured by both analytic and placement models when mapping a DL workload to edge node and its accelerator. 

These observations motivate the need for new analytic technique and systems mechanism for effectively sharing edge resources across multiple users and the devices when running AI inference workloads. In addressing these challenges, our paper make the following contributions: 1) We propose a two-tier architecture to deploy Deep Neural Network (DNN)-based inferencing workloads at the edge; 2) We use queuing model to capture the performance of the hardwares; 3) We design SLA-aware placement algorithm to deploy DNN workloads to edge cluster and 4) implement the system using Kubernetes; Finally, 5) we conduct experiment to validate our system. 

==> src/placement.tex <==
\section{Model-driven Resource Management }
\label{sec:slo}

In this section, we show how our analytic models can be used for edge resource management.

\subsection{Latency-aware Application Colocation}
Our queuing models predict the response time latency seen by two-tier inference applications in the presence of other co-located tenants (and performance interference which manifests itself as queuing delays). We can  use these analytic models to determine which applications to co-locate on each node and accelerator so that response time guarantees can be met. The heterogeneous nature of the cluster introduces additional challenges---servers can be equipped with multiple heterogeneous accelerators, and we must determine the optimal choice of accelerator for each tenant. 
%As we will show in \S \ref{sec:exp_resource_management} (see Figure \ref{fig:heterogeneous_profile}), 
The optimal choice depends on the DNN model, with the TPU offering faster execution times over the GPU for some DNN models, and vice versa (see Figure \ref{fig:heterogeneous_profile}). The response time also depends on the current utilization (load) on various accelerators and nodes. Finally, the application workload is itself heterogeneous comprising a mix of user-trained and AI-as-a-Service DNN models. The edge resource manager will need to consider these challenges when hosting multiple applications on each node.

We assume that  each application provides 1) the DNN model to be used for inference either using AI-as-a-Service or via a custom trained model, 2) the worst-case request rate $\lambda$, 3) the latency bound $\tau$ on to two-tier response time. For each new (incoming) application, our system needs to determine an appropriate node and type of accelerator (TPU or GPU) for execution. To determine the feasibility of co-locating the new application on each cluster node, along with existing tenants, the system estimates (i) the CPU response time of the frontend container and (ii) the GPU response time of the backend container  and (iii) the TPU response time of the backend container. It also verifies whether accelerator has enough memory to hold the DNN model and the execution run-time. Only nodes and accelerators where the sum of the CPU and GPU/TPU mean response time are less than the  desired target $R_i$ for all applications (i.e., current tenants and incoming one) are feasible candidates for co-locating the new application. The node and accelerator type with the lowest utilization change after placing the application is then chosen for the new application. 

In the case where the application uses AI-as-a-Service, we additionally consider a \emph{grouped} co-location strategy.  In grouped co-location, applications choosing the same pre-trained model are co-located (grouped) on the same server and accelerator.  In this case,  if the DNN model is already executing on the edge cluster (by being chosen by one or more prior applications), then we need to determine if the newly arriving application can be grouped with the existing ones. To do so, we aggregate the request rate $\lambda_i$ of all  grouped applications and use the analytic queuing model to determine the GPU and TPU response time of the backend container. 
%The two-tier response time and SLOs are used to determine a choice of node and accelerator, like before. A key advantage of the approach is that multiple applications share a backend container, allowing for memory savings and a higher degree of multi-tenancy on each edge servers.  
In the event the application cannot be grouped with any existing applications, it is placed onto a new server to start a new grouping. 

%\input{algorithms/placement}


%Our queuing models can be used to develop latency-aware placement algorithms that determine how to place an incoming customer onto a cluster of edge servers. In the context of cloud computing, virtual machine placement is viewed as a multi-dimensional Knapsack problem, where each server has multiple resources (e.g. CPU, memory) of a certain capacity and the objective is to maximize packing of virtual machines, each of which is given a certain allocation of CPU, memory, etc onto servers in the cluster. 

%Analogous to VM placement, our DNN model placement problem involves mapping frontend and backend containers onto edge servers such that the total resources allocated to all customers on that node is less than the node's capacity, and the latency SLO's of all customers are satisfied. Thus, we are given a cluster of edge servers that are equipped with a certain accelerator (e.g. EdgeTPU or GPU). Each incoming customer provides 1) the DNN model to be used for inference either using AI-as-a-Service or via a custom trained model, 2) the worse case request rate $\lambda$, 3) the SLO bound $\tau$ on to two tier response time (SLO). Our placement algorithms determine which node should run each model in order to meet its resource and SLO requirements. 

%\subsubsection{Individual Model Placement}

%For user-trained models, each DNN model should be placed individually onto the cluster. To do so, we need to compute the resource footprint of the DNN models for memory, CPU, GPU/TPU, then use a latency-aware variant of the bin packing problem to guide placement. We first compute the memory footprint of the DNN model, which is empirically estimated to be the sum of the memory size of the model and the memory footprint of the runtime system that executes the model. Given this memory footprint, only nodes with enough idle RAM to accommodate the frontend container and enough idle GPU/TPU memory to accommodate the backend container are feasible candidates for placement. 

%For each such node, we then use our analytic queuing model to estimate (i) the CPU response time of the frontend container and (ii) the GPU/TPU response time of the backend container. Note that when computing the backend response time, we need to consider current DNN models that are already executing on that node (since the GPU/TPU is shared across all resident applications). Only nodes where the sum of the CPU and GPU/TPU mean response time are less than the SLO threshold for all applications (including current applications and incoming one) are feasible nodes. Any node from the feasible set can be chosen, for example, using best-fit or least-loaded strategy.

%\subsubsection{Grouped Model Placement}

%While the above individual placement algorithms are suitable for placement of user-trained DNN models, a grouped placement strategy is desirable for placement of AI-as-a-Service applications. In grouped placement, applications choosing the same pre-trained model are co-located (grouped) on the same server. However, since each node has a finite resource capacity, the number of customers who can be grouped onto a node is determined by our analytic queuing models. In this case, each incoming customer chooses from a list of pre-trained models. If no previous customer has chosen this model, an idle or lightly utilized server is chosen for this DNN model. If the DNN model is already executing on the edge cluster (by being chosen by one or more prior customers), then we need to determine if the newly arriving customer can be grouped with the existing ones. To do so, we aggregate the request rate $\lambda_i$ of all customers and use the analytic queuing model to determine the GPU/TPU response time of the backend container. Next, the placement techniques check if there is enough idle RAM to accommodate one more frontend container. If so, it also determines CPU response time of the frontend customer for the new application. The application can be grouped onto this node if the sum of the backend and frontend response time satisfies SLO threshold of all applications, and available RAM is sufficient to accommodate the new application\footnote{Since the backend is shared, there is no change in the memory usage of the backend container.}. If there are inadequate resources to meet the SLO, the customer cannot be grouped on the current server and is placed onto a new idle server to start a new grouping. 


%\footnote{It is also possible to live migrate the containers to the new server. However, our current prototype does not use live migration due to the lack of a mature live migration technique in Kubernetes.}
 



%If an application experiences an increase in its incoming request rate $\lambda_i$, it may experience SLO violations and also cause SLO violations for other customers that share the GPU/TPU on that node. Such a hotspot can be mitigated through dynamic migration, where the overloaded application is moved to a new edge node with sufficient idle resources to handle the increased workload. 

%Our migration algorithm includes a monitoring component that continuously monitors the end-to-end mean two-tier response time for each application over a moving time window. It also tracks the observed request rate $\hat{\lambda_i}$ for each application.

%If SLO violation is observed on any node, the application whose observed request rate $\hat{\lambda_i}$ exceeds the estimated rate $\lambda_i$ during initial placement is flagged as overloaded. Our analytic queuing model is invoked to determine a new placement for this application. A new estimate for incoming workload is used based on the higher observed arrival rate in the queuing model. Once a new node has been chosen for this application using the individual model placement algorithm above, the frontend, and backend containers are migrated to that node and subsequent requests are directed to the new node\footnote{It is also possible to live migrate the containers to the new server. However, our current prototype does not use live migration due to the lack of a mature live migration technique on Kubernetes.}. This results in the mitigation of the hotspot on the previous node.

\subsection{Ibis Implementation}
\begin{figure}
	\centering
	\captionsetup{belowskip=-14pt}
	\includegraphics[width=0.25\textwidth]{imgs/impl_overview}
	\caption{Ibis implementation overview}
	\label{fig:impl_overview}
\end{figure}

We have implemented a prototype of our system, named Ibis, using Kubernetes on a  custom-built edge cluster of ten nodes, each comprising a Jetson Nano GPU, 4 GB of RAM, and quad-core ARM processor. We use a similar ten node cluster equipped with USB edge TPUs for our TPU experiment. Our cluster also contains a Dell PC with 3.2 GHZ i7-8700 processor, 16 GB RAM, and Geforce-GTX-1080 GPU. All machines are connected via a gigabit ethernet switch and run Linux Ubuntu 18.04. Further, each Jetson Nano runs CUDA 10.2, cuDNN 8, and TensorRT 7.1.3 while the PC runs CUDA 11, cuDNN 7.6.5, and TensorRT 7.1.3. All machines are virtualized using Docker 19 and managed by Kubernetes 11; gRPC 1.31 is used for inter-communication.

Figure \ref{fig:impl_overview} depicts Ibis system overview. Our prototype currently runs DNN models in TensorRT engine format for GPU and quantized \texttt{tflite} format for EdgeTPU. For AIaaS models, Ibis first retrieves its resource requirements (e.g. memory, service time) using a pre-profile table. On the other hand, in case of User-Supplier models (provided in ONNX format), we then compile and profile it on an idle node and save the result back to the profile table for future use. Our application containers  are deployed as Kubernetes \texttt{Deployment}, and we use Kubernetes \texttt{Service} to route network traffic. Ibis collects node resource status and chooses a node and device using our analytic models and scheduling strategies. Finally, Ibis deploys incoming workload to target node and device via Kubernetes interface. Source code for our prototype is available on github \emph{(URL blinded)}.



\subsection{Experimental Evaluation of Model-driven Resource Algorithms}\label{sec:exp_resource_management}
%\begin{figure}
	%\centering
	%\includegraphics[width=0.4\textwidth]{imgs/heterogeneous_profile.pdf}
	%\caption{Normalized service time for various DNN models.}
	%\label{fig:heterogeneous_profile}
%\end{figure}


\input{imgs-latex/placement_figures}

%Having evaluated the efficacy of our queuing models, 
In this section, we experimentally evaluate our cluster resource management techniques on a  edge cluster using realistic workloads. To do so, we deploy Ibis on our 10 node edge cluster and use the  trace workloads discussed below for our experiments.


\subsubsection{Trace Workloads} The  trace workload for each IoT application is constructed using a sequence of images from the ImageNet dataset \cite{imagenet}.   Further, to construct a mix of IoT applications  to run on our edge cluster,  we use the public Azure trace \cite{Azure-traces} to construct a realistic mixes of containerized applications of varying sizes.  To do so, we analyze the distribution of VM sizes  (CPU utilization and memory footprint) 
in the Azure trace and use them to generate the utilization and model size of our DNN-based applications. We categorize VMs as small ($<$2GB), medium (2-8GB), and large ($>$8GB) and find that proportions of small, medium and large applications is 47\%, 33\%, and 20\% respectively.   The mix of small, medium and large DNN models housed on the edge cluster is chosen in the same proportion.  Finally, models in the same category are chosen evenly. 

We uses this Azure trace to generate an arrival trace of DNN applications that require placement on our cluster. Each arriving application is chosen from the above DNN types and is associated with a response time constraint $R_i$, and worst case request rate $\lambda$. 



%\textcolor{blue}{\subsubsection{DNN profiling}\label{sec:dnn} 
%As mentioned earlier, to enable performance estimates, models are profiled on an idle node. For GPUs, models are compiled using TRT compiler. For TPUs, models are first quantized to 8-bit integers, then compiled using Edge TPU compiler. The output of the profiling process include the service time, static model size, memory foot-print, and context switch overhead. As mentioned in \S \ref{sec:edge_tpu_device} TPU devices are limited in memory and executing different models concurrently incurs a non-negligible context switch overhead. Figure \ref{fig:tpu_switch_overhead} shows the memory allocations (on-chip and off-chip) and context switch overhead. This overhead  is proportional to on-device memory size but independent of the model that was previously loaded on the device---unlike CPU context switches, there is no DNN state that needs to be saved back to RAM (since inference execution does not change the model parameters). On the other hand, GPUs are have much more memory and context switch overhead is negligible. 
%}
%\textcolor{blue}{Figure \ref{fig:heterogeneous_profile} highlights the performance of models on TPUs and GPUs. As shown, models that entirely fit on the TPU (such as MobileNet) executes faster than when placed on the TPU while models that have a large off-chip memory (such as Inception) executes faster on the GPU. The main reason is that larger models processing includes memory swaps for the TPU that increases the processing time. Full details on service time of different models are available in Table \ref{tab:all-models} in the Appendix.}
\subsubsection{DNN profiling} \label{sec:DNN_profiling} We start with profiling target DNNs. We perform this on an idle node to avoid any interference. We measure memory footprint, service time on GPU, service time on Jetson Nano GPU, service time, and switch overhead on EdgeTPU. 
%and the detailed results are shown in table \ref{tab:all-models} in Appendix. 
Figure \ref{fig:heterogeneous_profile} shows the normalized execution time of various models. Interestingly, the figure shows that some DNN models run faster on the TPU than the GPU, and while others run faster on the GPU.
%As shown in the figure, the relative service time between Nano GPU and EdgeTPU varies across DNNs. 
This is because the EdgeTPU is an ASIC designed specifically for DNN inference and has higher operations per second than more general-purpose GPU device. But it has a small (i.e. 8 MB) device, or on-chip memory. To run models with memory footprint larger than this limit, it employs host, or off-chip memory to store the extra model parameters. Since accessing off-chip memory is much slower than accessing on-chip memory, in general, larger DNNs  have worse performance than smaller DNNs on EdgeTPU. On the other hand, GPU does not have this problem as it stores all DNN runtime and parameters on device memory and we would prefer to place those TPU-unfriendly DNNs on GPU. Thus, to achieve maximal sharing, a heterogeneity-aware policy is needed. 

Moreover, DNN on-chip memory size also affects the switch overhead on EdgeTPU. When performing context switch, EdgeTPU needs to load the on-chip part of the incoming model into the device memory. As a result, the context switch overhead has a linear relationship with DNN on-chip memory size as shown in figure \ref{fig:tpu_switch_overhead}.  Our  results shows that neither the TPU or GPU is optimal for all DNN models and  the optimal choice will depend on the characteristics of each  model. This result also motivates our heterogeneous placement technique discussed in Sec XXXXXXXXXXXX.



\subsubsection{Efficacy of co-location algorithms} We first conduct an experiment to co-locate a mix of IoT applications 
on  the cluster using AI-as-a-Service. In this experiment, we compare three policies :1) a latency-oblivious policy that only looks at memory footprint for placement (i.e. using a knapsack approach); 2) our latency-aware grouped placement policy that select feasible nodes but randomly choose device type; 3) our latency \& heterogeneity-aware grouped placement policy that selects the optimal accelerator type that offers lowest service time. Figure~\ref{fig:edgetpu-slo} depicts our results. As shown, the latency-oblivious policy see latency violations even with a small number of co-located applications, and the number of applications seeing violation increase with more customer arrivals. When we try to load more than 50 customers with latency-oblivious policy, the system crashes. In contrast, our latency-aware policy is able to place 61 customers on to the cluster, with no latency violation for any of the customers. Furthermore, our latency \& heterogeneity-aware policy is able to place 70 customers on to the cluster without any latency violations. These validate that Ibis is able to maximize resource sharing while maintaining response time guarantees.

\subsubsection{Multi-tenant colocation  for dynamic workloads} Next, we conduct an experiment to compare the degree of sharing achieved using   AI-as-a-Service applications, user-trained models, and a mix of both. 
Figure \ref{fig:placement_user_iaas} shows the number of applications that can be placed on the cluster in each case; since AI-as-a-Service customers share backend resources, they can achieve a greater degree of resource sharing. The figure shows that each Jetson Nano node can hold only 2 to 3 DNN models since TensorRT run time takes around 800 MB aside from the models' actual memory requirements. %(see table \ref{tab:all-models}).
However, in the AI-as-a-Service, the system can host double the number of customers since backend sharing amortizes the memory footprint of the TensorRT runtime. Customers need only a small frontend container due to backend sharing, allowing for better GPU utilization by hosting more customers. On the other hand,  in the user-trained case, the memory limit on a node is reduced once 2-3 models are placed, and additional DNN models cannot be placed even though the GPU is underutilized. Finally, the mixed workload achieves co-location performance that lies between the two.
%hosts the same number of backend containers and user-trained but less frontend than AI-as-a-Service.


%Next, we compare resource management of AI-as-a-Service hosting with user-trained hosting. We use the same arrival trace to first place all customers using the AI-as-a-Service hosting model, and then use the same trace assuming all models are user-trained. Figure \ref{fig:placement_user_iaas} shows the number of customers that can be placed on the cluster in each case; since AI-as-a-Service customers share backend resources, they can achieve a greater degree of resource sharing. The figure shows that each Jetson Nano node can hold only 2 to 3 DNN models since TensorRT run time takes around 800 MB aside from the models' actual memory requirements (see table \ref{tab:models}). However, in the AI-as-a-Service, the system can host double the number of customers since backend sharing amortizes the memory footprint of the TensorRT runtime. Customers need only a small frontend container due to backend sharing, allowing for better GPU utilization by hosting more customers. On the otherhand,  in the user-trained case, the memory limit on a node is reduced once 2-3 models are placed, and additional DNN models cannot be placed even though the GPU is underutilized.  This result shows that in resource constrained  edge clusters, greater resource sharing allows for a higher degree of packing, and better cluster utilization.

%We further study the performance of our SLO-aware user-trained placement policy versus best-fit, first-fit, and worst-fit SLO agnostic placement policies for the same experiment in Figure~\ref{fig:placement_user_iaas}. Figure \ref{fig:placement_nano_sla} shows the SLO violation rate  for different placement policies. As shown, the violation rate is high for all SLO agnostic policies. Even with a low number of customers in the system, we saw significant SLO violations. On the other hand, the case of AI-as-a-Service with model unaware placement yielded a huge increase in DNN models packed on the GPUs leading to 100\% SLO violation. Appendix \ref{apx:placement_1080} shows more placement results.

\subsubsection{Evaluation of hotspot migration with token bucket} Finally, we conduct an experiment to demonstrate the efficacy of hotspot mitigation with token bucket. We start the experiment with the system moderately loaded with two DNN models --- EfficientNet-S and MobileNetV2. We then increase the request rate of EfficientNet-S beyond the placement time estimate. As shown in figure \ref{fig:migration}, the workload increase causes the response time of EfficientNet-S to exceed the latency threshold but does not affect the MobileNetV2 because of the token bucket. Our system monitors the response time seen by customers and triggers a migration when violations are observed. The overloaded application is migrated to a new node with sufficient idle capacity, causing the response time of the overloaded application to fall below the latency violation threshold. This experiment shows the ability of our techniques to mitigate hotspots dynamically.

==> tables/context_switch.tex <==
\begin{table*}[t]
\begin{tabular}{l|lllll}
\textbf{}        & EffiNet-S & EffiNet-M & EffiNet-L & Inception V4 & SSD mobilenet V2 \\ \hline 
EffiNet-S        & 0.00      & 17.40     & 17.39     & 17.46        & 17.40            \\
EffiNet-M        & 17.59     & 0.00      & 17.62     & 17.69        & 17.65            \\
EffiNet-L        & 13.53     & 13.61     & 0.00      & 13.66        & 13.62            \\
Inception   V4   & 15.24     & 15.47     & 15.36     & 0.00         & 15.40            \\
SSD mobilenet V2 & 17.62     & 17.72     & 17.63     & 17.67        & 0.00            
\end{tabular}
\caption{Context switch overhead matrix, where cell $i, j$ represents the context switch overhead of model $i$ when running model $j$ prior to it.}
\label{tab:context_switch}
\end{table*}

==> tables/edgetpu_models.tex <==
\include{tables/merged_models}% Please add the following required packages to your document preamble:
% \usepackage{multirow}

\begin{table*}[t]
\resizebox{\textwidth}{!}{%
\begin{tabular}{|l|l|l|l|l|l|l|}
\hline
Model            & Scale & On-chip (MB) & Off-chip (MB) & Size (MB) & Service time (ms) & Overhead (ms) \\ \hline
\multicolumn{7}{|c|}{Image Classification Models}                                                       \\ \hline
Efficientnet-S   & S     & 6.56         & 0.00          & 6.56      & 9.83              & 17.33         \\ \hline
Efficientnet-M   & M     & 6.74         & 1.59          & 8.33      & 15.64             & 17.62         \\ \hline
Efficientnet-L   & L     & 5.17         & 7.13          & 12.3      & 37.72             & 13.59         \\ \hline
Mobilenet v1     & S     & 4.21         & 0.00          & 4.21      & 4.56              & 11.62         \\ \hline
Mobilenet v2     & S     & 3.75         & 0.00          & 3.75      & 4.87              & 10.43         \\ \hline
Inception v3     & L     & 5.67         & 17.69         & 23.36     & 49.97             & 14.65         \\ \hline
Inception v4     & L     & 6.03         & 36.13         & 42.16     & 98.11             & 15.17         \\ \hline
\multicolumn{7}{|c|}{Object Detection Models}                                                           \\ \hline
SSD Mobilenet v1 & M     & 6.7          & 0.00          & 6.7       & 22.14             & 17.88         \\ \hline
SSD Mobilenet v2 & M     & 7.1          & 0.00          & 7.1       & 25.94             & 16.36         \\ \hline
\end{tabular}
}
\caption{DNNs for EdgeTPU.}
\label{tab:edgetpu-models}
\end{table*}



==> tables/merged_models.tex <==

\begin{table}[h]
\centering
\resizebox{\textwidth}{!}{%
\begin{tabular}{|c|c|c|c|c|c|c|c|c|c|c|c|}
\hline
  \multicolumn{5}{|c|}{General Properties} &
  \multicolumn{3}{c|}{GPU Properties} 
  & \multicolumn{4}{c|}{TPU}\\ \hline
Models &
  Scale &
  Input Shape &
  Parameters &
  \begin{tabular}[c]{@{}c@{}}FLOPS \\ (GF)\end{tabular} &
  \begin{tabular}[c]{@{}c@{}}Size \\ (MB)$^*$\end{tabular} &
  \begin{tabular}[c]{@{}c@{}}Memory \\  (MB)$^*$\end{tabular} &
  \begin{tabular}[c]{@{}c@{}}Inference \\ Time (ms)$^*$\end{tabular} &
  \begin{tabular}[c]{@{}c@{}}Size \\ (MB)\end{tabular} &
  \begin{tabular}[c]{@{}c@{}}Memory \\  On-chip + Off-chip \\(MB)\end{tabular} &
  \begin{tabular}[c]{@{}c@{}}Inference \\ Time (ms)$^*$\end{tabular} &
  \begin{tabular}[c]{@{}c@{}}Overhead \\ Time (ms)$^*$\end{tabular} \\ \hline
\multicolumn{12}{|c|}{Classification Models}                                         \\ \hline
AlexNet         & S & {[}N, 3, 224, 224{]} & 62M     & 0.7    & 138 & 992  & 14.18  &    -   &    -   &    -   &   - \\ \hline
GoogleNet       & S & {[}N, 3, 224, 224{]} & 6 M     & 2      & 39  & 893  & 13.37  &    -   &    -   &    -   & -    \\ \hline
InceptionV3     & M & {[}N, 3, 224, 224{]} & 24 M    & 6      & 81  & 836  & 30.56  &   24.03    &  5.65 + 17.85  &  49.27     &   14.88    \\ \hline
MobileNetV2     & S & {[}N, 3, 224, 224{]} & 3.5 M   & 0.6    & 22  & 1130 & 13.02  &   4.05    &    3.88 + 0   &   4.43    &    10.71   \\ \hline
ResNet18        & S & {[}N, 3, 224, 224{]} & 12 M    & 1.8    & 69  & 930  & 10.83  & 11.46  & 7.18 + 4.09     &    14.31  &   18.93  \\ \hline
ResNet34        & M & {[}N, 3, 224, 224{]} & 21.2 M  & 3.6    & 155 & 1044 & 19.51  & 21.28  & 7.18 + 13.83    &  38.92  &  18.74   \\ \hline
ResNet50        & M & {[}N, 3, 224, 224{]} & 26 M    & 3.8    & 106 & 965  & 29.2   & 24.9   & 6.33 + 18.35    &   49.61     &   16.48     \\ \hline
ResNet101       & L & {[}N, 3, 224, 224{]} & 44.5 M  & 7.6    & 247 & 1135 & 50.32  & 43.43  & 6.34 + 36.71    &  95.72   &   16.52  \\ \hline
EfficientNet-b0 & S & {[}N, 3, 224, 224{]} & 5.3 M   & 0.4    & 30  & 1168 & 26.03  & 6.72   & 4.6 + 1.46      &   29.91     &   11.88   \\ \hline
EfficientNet-b1 & S & {[}N, 3, 240, 240{]} & 7.8 M   & 0.7    & 42  & 1184 & 41.32  & 9.84   & 4.11 + 4.84     &   62.97  &   11.05    \\ \hline
EfficientNet-b2 & M & {[}N, 3, 260, 260{]} & 9.2 M   & 1      & 49  & 1196 & 49.58  &   -    &  -  &    -  &  -   \\ \hline
EfficientNet-b3 & M & {[}N, 3, 300, 300{]} & 12 M    & 1.8    & 77  & 1229 & 81.67  &   -    &  -  &    -  &  -   \\ \hline
EfficientNet-b4 & L & {[}N, 3, 380, 380{]} & 19 M    & 4.2    & 124 & 1042 & 166.15 &   -    &  -  &    -  &  -   \\ \hline
EfficientNet-b5 & L & {[}N, 3, 456, 456{]} & 30 M    & 9.9    & 180 & 180  & 337.44 &   -    &  -  &    -  &  -   \\ \hline
DenseNet121     & L & {[}N, 3, 224, 224{]} & 7.2 M   & 3      & 50  & 910  & 30.14  &   9.34 &  7.16 + 2.95    &  16.88   &   15.18  \\ \hline
DenseNet201     & L & {[}N, 3, 224, 224{]} & 20 M    & 4      & 103 & 964  & 89.11  &  23.27    & 6.45 + 15.78    &  49.15  &  16.76  \\ \hline
VGG16           & L & {[}N, 3, 224, 224{]} & 138 M   & 16     & 407 & 1275 & 86.36  &  132.34  & 5.61 + 126.5    &  333.37  &   14.83  \\ \hline
VGG19           & L & {[}N, 3, 224, 224{]} & 144 M   & 20     & 463 & 1333 & 99.19  &  137.42      &    5.61 + 131.58    &  346.78  &     14.7  \\ \hline
\multicolumn{12}{|c|}{Object Detection Models}                                       \\ \hline
YoloV3          & L & {[}N, 3, 416, 416{]} & 62 M    & 65.88  & 617 & 1501 & 190.24 &   -    &  -     &   -    &  -     \\ \hline
YOLO-tinyV4     & M & {[}N, 3, 416, 416{]} & 6.06 M  & 6.91   & 75  & 938  & 23.79  &   -    &  -     &   -    &  -     \\ \hline
YoloV4          & L & {[}N, 3, 608, 608{]} & 64.43 M & 128.46 & 445 & 1329 & 407.91 &   -    &  -     &   -    &  -     \\ \hline
SSD Mobilenet v1 & M &    {[}N, 3, 300, 300{]} & 6.8 M &  1.2  &  -   &   -   & - & 6.7    &  6.7 + 0.00   & 22.14 & 17.88 \\ \hline
SSD Mobilenet v2 & M & {[}N, 3, 300, 300{]} &  4.3 M   &  0.8  &  -  & -  & -  & 7.1    &  7.1 + 0.00   & 25.94 & 16.36 \\ \hline
\end{tabular}%
}
\caption{DNN characteristics for GPU and TPU (Values are based on Jetson Nano with FP16, different configuration might yield different values).}
\label{tab:all-models}
\end{table}

==> tables/relative_error.tex <==
\begin{table}[]

\resizebox{\columnwidth}{!}{
\begin{tabular}{l|llll}
Models                                                            & 30\%-45\% & 45\%-60\% & 60\%-75\% & Max    \\ \hline
Efficientnet-S                                                    & 0.0018    & 0.0310    & 0.0488    & 0.0488 \\
Efficientnet-M +   Efficientnet-S                                 & 0.0989    & 0.0445    & 0.0993    & 0.0993 \\
Inception V4 + Mobilenet V2                                       & 0.0499    & 0.1077    & 0.0409    & 0.1077 \\
Inception V3 + SSD   Mobilent V2                                  & 0.0681    & 0.0325    & 0.0476    & 0.0681 \\
Efficientnet-L + Inception V3 + Inception V4                      & 0.0308    & 0.0498    & 0.0441    & 0.0498 \\
Efficientnet-S   + Mobilenet V1 + Mobilenet V2 + SSD Mobilenet V2 & 0.0398    & 0.0493    & 0.0323    & 0.0493
\end{tabular}
}

\caption{The table shows the maximal relative error of our queuing model prediction under the various model combinations and system utilization.}
\label{tab:edgetpu-relerror}
\end{table}
